A Framework for Creative-Visualization Opportunities Workshops

Applied visualization researchers often work closely with domain collaborators to explore new and useful applications of visualization. The early stages of collaborations are typically time consuming for all stakeholders as researchers piece together an understanding of domain challenges from disparate discussions and meetings. A number of recent projects, however, report on the use of creative visualization-opportunities (CVO) workshops to accelerate the early stages of applied work, eliciting a wealth of requirements in a few days of focused work. Yet, there is no established guidance for how to use such workshops effectively. In this paper, we present the results of a 2-year collaboration in which we analyzed the use of 17 workshops in 10 visualization contexts. Its primary contribution is a framework for CVO workshops that: 1) identifies a process model for using workshops; 2) describes a structure of what happens within effective workshops; 3) recommends 25 actionable guidelines for future workshops; and 4) presents an example workshop and workshop methods. The creation of this framework exemplifies the use of critical reflection to learn about visualization in practice from diverse studies and experience.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
last modified by Bernhard Finkbeiner, July 5, 2010

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored by
the IEEE Visualization & Graphics Technical Committee (VGTC).

The only conferences that use the 'journal' document option:
- IEEE Visualization Conference (Research and Application Papers Only)
- IEEE Information Visualization Conference (Research and Application
Papers Only)

It contains 13 files:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed,
                  somewhere in the TeX search path
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
sample.eps      - an image used by the example paper
sample.pdf      - its PDF version
template-journal*.pdf    - an example proper pdf output in default
                          conference mode, with and without teaser
CypressView.eps - teaser image
CypressView.pdf - its PDF version
makefile     - makefile including bibtex compilation and proper PDF
                generation

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We
suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create
a file called 'template.pdf'. Please make sure, that its layout is
identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process
manually.  Below are a list of available options that may be passed to
make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> boxes/defining-a-theme.tex <==
\begin{tcolorbox}[floatplacement=t,float,title=Defining a {\it Visualization} Workshop Theme]
The workshop theme summarizes the central topic of the workshop. Visualization creativity requirements workshops differ from workshops in other domains as their themes should aspire to:
\begin{itemize}[noitemsep,nolistsep]
\item {\it Focus on interesting visualization opportunities} that identify a real need of analysts that exhibit the appropriate data location and task clarity~\cite{Sedlmair2012}.
\item {\it Identify relevant analysts and domain data,} necessary to invite participants and tailor workshop methods to explicitly incorporate questions about data, analysis, and visualization.
\item {\it Target results that benefit all project stakeholders,} including researchers, to better understand domain challenges, and collaborators, to think creatively about how they make sense of data.
\end{itemize}
\end{tcolorbox}

==> boxes/fostering-creativity.tex <==
\begin{tcolorbox}[floatplacement=t,float,title=Fostering Creativity with CACTI Factors]
Reflecting on our experience, and reviewing relevant literature~\cite{Nickerson1999,Osborn1953,Sawyer2003,Sawyer2006,Shneiderman2005}, reveals a number of key factors that influence the engagement and creativity of workshop participants: fostering, maintaining, and potentially varying the levels of collegiality, agency, challenge, trust and interest associated with each, as well as the focus on visualization and data in the context of the specialist domain. To help us remember these factors, we term them {\bf CACTI factors}: 
\begin{itemize}[noitemsep,nolistsep]
\item(\textbf{C})ollegiality -- the degree to which communication and collaboration are encouraged and occur;
\item(\textbf{A})gency -- the sense of participant ownership in workshop outcomes and research project;
\item(\textbf{C})hallenge -- the barrier of entry to, and likelihood of success in workshop methods; 
\item(\textbf{T})rust --  the confidence that participants have in the methods, the design process, and the researcher's visualization expertise; 
\item(\textbf{I})nterest -- the amount of attention, energy and engagement to workshop methods;
\item\textbf{+} -- ~other \emph{relevance} factors that can effect: the levels of engagement with \emph{data}, \emph{visualization} and the \emph{domain} in which collaborators are working.
\end{itemize}
The CACTI factors are neither independent, consistent, nor measurable. The extent to which they are fostered depends upon the context in which they are used, including various characteristics of the workshop group - often unknown in advance, though perhaps detectable by facilitators. And yet, maintaining appropriate levels of the factors likely helps workshops to inspire and engage participants while creating useful output and establishing lasting rapport among researchers and their collaborators.
\end{tcolorbox}

==> boxes/getting-creative.tex <==
\begin{tcolorbox}[floatplacement=b,float,title=Getting Creative with Workshop Design]
The ideas presented in this paper are a starting point for thinking about workshop design. We are excited by the potential for researchers to think creatively about what methods to use and how to tailor them for visualization creativity workshops. In reporting on the effecitveness of methods, we encourage answering the following questions as exemplified by Goodwin et al.~\cite{Goodwin2013}:
\begin{itemize}[nolistsep,noitemsep]
\item {\it What methods were used?}
\item {\it What was the intended result of each method?}
\item {\it What was the real result of each method?}
\item {\it How useful was the method result?}
\end{itemize}


To illustrate the workshop structure, our Supplemental Material includes an example workshop plan which has been adapted and validated in three projects [\ref{wor:eon},~\ref{wor:graffinity},~\ref{wor:cp}]. We include this plan as a starting point for researchers to consider workshops in their own projects.
\end{tcolorbox}

==> boxes/learning-from-experience.tex <==
\begin{tcolorbox}[floatplacement=t,float,title=Learning from Experience with Critically Reflective Practice]

In applied visualization, reflection transforms engineering into research~\cite{Sedlmair2012}. We use a methodology of critically reflective practice~\cite{Brookfield1998} to analyze our collective experience. Due to the nature of reflective analysis, we recognize that the framework is not exhaustive, predictive, nor objective. Nevertheless, {\it the framework is consistent with our experience, grounded in existing theory, and likely useful for future visualization research.}

\end{tcolorbox}


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> tables/guidelines.tex <==
\begin{table}
    \centering
    \begin{tabular}{|p{0.9\linewidth}|}
    \hline
    Define the problem. \\
    Recruit diverse and creative participants. \\
    Design within constraints. \\
    Test, test, test. \\
    \hline
    Set the stage --- engage.\\
    Encourage self-expression. \\
    Elicit relevant ideas. \\
    Explore, then focus. \\
    Create physical artifacts \\
    Balance activity with rest \\
    Mix it up.\\
    Transition smoothly. \\
    Reflect to hep analysis.\\
    Promote continued creative collaboration. \\
    Ask for feedback. \\
    \hline
    Prepare to execute. \\
    Limit distractions. \\
    Get out of the way. \\
    Guide gently. \\
    Be flexible. \\
    Adapt tactically. \\
    Record ideas collectively and with context. \\
    \hline
    Allocate time. Soon. \\
    Create a corpus. \\
    Analyze with an open mind. \\
    Act creatively.\\
    Revisit, reflect, and report on the workshop. \\
    \hline
    \end{tabular}
    \caption{Summary of guidelines for future workshops.}
    \label{tab:design-considerations}
\end{table}


==> tables/trash/design-considerations.tex <==
\begin{table}
    \small
    \centering
    \begin{tabular}{|m{0.07\linewidth}|p{0.8\linewidth}|}
    \hline
    ID & Consideration \\
    \hline
    \des{des:context}{} & Effective openings establish context and promote group creativity. \\
    \des{des:interpersonal}{} & Interpersonal introductions can support communication and creativity. \\
    \des{des:leading}{} & Allowing participants to lead in the opening may increase engagement. \\
    \des{des:beware}{} & Passive methods in the opening may discourage participation. \\
    \hline
    \des{des:ideaspace}{} & The ideaspace focuses on data, analysis, automation, and visualization.  \\
    \des{des:diverge-converge}{} & Diverge-converge cycles can develop the ideaspace.  \\
    \des{des:cascading}{} & Methods have cascading influences on the ideaspace.  \\
    \des{des:externalize}{} & Effective methods externalize ideas.  \\
    \des{des:post-it}{} & Post-it notes are particularly useful for externalization.  \\
    \des{des:passive}{} & Passive methods can support creativity.  \\
    \des{des:visualization-analogies}{} & Visualization analogies can excite and engage participants.  \\
    \des{des:convergence}{} & Convergence can conclude methods and the workshop core. \\
    \hline
    \des{des:closing}{} & Closing discussions can promote reflection and validation \\
    \des{des:feedback}{} & Effective closings can prepare participants to give feedback. \\ 
    \des{des:action}{} & Identifying the next steps of action can provide validation. \\
    \hline
%% JD \des{des:resources}{} & Existing resources describe a plethora of methods. \\
%% JD \des{des:tailor}{} & Methods can be tailored to explore visualization and data analysis. \\
%% JD \des{des:support}{} & Methods can be evaluated as creativity support tools.\\
    \des{des:resources}{} & Existing resources describe a plethora of methods. \\
    \des{des:select}{} & Methods should be selected in consideration of key characteristics (CACTI). \\
    \des{des:adapt}{} & Methods can be adapted to explore data, visualization and domain. \\
    \des{des:support}{} & Methods can be evaluated as creativity support tools.\\

    \hline
    \end{tabular}
    \caption{Summary of the workshop design considerations.}
    \label{tab:design-considerations}
\end{table}


==> tables/trash/method-characteristics.tex <==
\begin{table}
    \small
    \centering
    \begin{tabular}{|m{0.7\linewidth}|m{0.03\linewidth}|m{0.03\linewidth}|m{0.03\linewidth}|}
        \hline
        \textbf{Method Characteristics} & \textbf{Op.} & \textbf{Co.} & \textbf{Cl.} \\
        \hline
        \emph{Agency} --- providing a feeling of ownership, responsibility, or ability to act by encouraging self-expression and choice.~\cite{Brooks-Harris1999}. & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ \\
        \hline
        \emph{Communication} --- encouraging the sharing of ideas by encouraging trust, necessary for synergistic group creativity~\cite{Sawyer2003}. & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ \\
        \hline
        \emph{Data, analysis and automation} --- promoting thinking about relevant topics to the design study. & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ \\
        \hline
        \emph{Visualization} --- exploring the use of visualizations through sketching, demonstrations, or visual language.  & $\CIRCLE$ & $\CIRCLE$ & $\CIRCLE$ \\
        \hline
        \emph{Exploration} --- promoting analysis of new emergent ideas by encouraging creativity~\cite{Nickerson1999}. & $\Circle$ & $\CIRCLE$ & $\Circle$ \\
        \hline
        \emph{Generation} --- creating new ideas to support exploration of a broad ideaspace, also referred to as \emph{divergent} thinking ~\cite{Osborn1953}. & $\Circle$ & $\CIRCLE$ & $\Circle$\\
        \hline
        \emph{Evaluation} --- winnowing the broad ideaspace into a narrow set of promising ideas, also referred to as \emph{convergent} thinking~\cite{Osborn1953}. & $\Circle$ & $\CIRCLE$ & $\CIRCLE$ \\
        \hline
        \emph{Externalization} --- representing ideas in physical medium, supporting communication and creativity~\cite{Sawyer2006}. & $\Circle$ & $\CIRCLE$ & $\Circle$ \\
        \hline 
        \emph{Connection} --- revisiting concepts by connecting methods through artifacts or ideas. & $\Circle$ & $\CIRCLE$ & $\CIRCLE$ \\
        \hline
        \emph{Incubation} --- providing downtime to allow for conscious and unconscious thought~\cite{Sawyer2006}. & $\Circle$ & $\CIRCLE$ & $\Circle$\\
        \hline
        \emph{Reflection} --- promoting metacognition and analysis of experience to generate insights~\cite{Boud1985} &  $\Circle$ & $\CIRCLE$ & $\CIRCLE$\\
        \hline
        \emph{Validation} --- encouraging continued collaboration by demonstrating the value of ideas, time, or energy committed~\cite{Hamilton2016}. & $\Circle$ & $\CIRCLE$ & $\CIRCLE$ \\
        \hline
    \end{tabular}
    \caption{Twelve characteristics of methods that connect to three phases of the workshop structure. Although all characteristics are important throughout the workshop ($\Circle$), our successful workshops emphasized certain characteristics during the opening, core, and closing ($\CIRCLE$).}
    \label{tab:method-characteristics}
\end{table}


==> tables/trash/methods.tex <==
\begin{table}
    \small
    \centering
    \begin{tabular}{|m{0.9\linewidth}|}
        \hline
        \textbf{Methods} \\
        \hline
        \textbf{\emph{Analogy Introduction}} --- a playful introduction to prime analogical thinking e.g., \emph{``if you were to describe yourself as an animal, what would you be?''}~[\ref{wor:eon}] \\
        \hline
        \textbf{\emph{Constraint Removal}} --- identifying constraints around current ideas, considering the removal of each constraint, and imagining  what would be possible~\cite{Jones2008}. \\ 
        \hline
        \textbf{\emph{Brainstorming}} --- unstructured ideation, \emph{``using the \emph{brain} to \emph{storm} a creative problem...through freewheeling generation of ideas''} \cite{Osborn1953}. \\
        \hline
        \textbf{\emph{Clustering}} --- grouping ideas into meaningful sets with descriptive titles\\
        \hline
        \textbf{\emph{Storyboarding}} --- creating a graphical depiction of a narrative ~\cite{Truong2006}\\
        \hline
        \textbf{\emph{Visual Improv.}} --- rapidly sketching concepts of increasingly complexity e.g., a line, a shape, a mountain, a pet, a mode of transportation, a dangerous mountain, a helpful pet, a friendly mode of transportation ... \\ 
        \hline
        \textbf{\emph{Visual Analogies}} --- displaying a curated set of visualization and encouraging ideation about how aspects of the visualizations may apply to a domain~\cite{Koh2011} \\
        \hline
        \textbf{\emph{Wishful Thinking}} --- prompted with a scenario, generating ideas in response to: What would you like to know? What would you like to see? What would you like to do? \\
        \hline
    \end{tabular}
    \caption{}
    \label{tab:methods}
\end{table}


==> tables/trash/recommendations.tex <==
\begin{table}
    \small
    \centering
    \begin{tabular}{|m{0.06\linewidth}|p{0.8\linewidth}|}
    \hline
    ID & Recommendation \\
    \hline
    \rec{rec:theme}{} & Articulate a mutually beneficial workshop theme. \\
    \rec{rec:participants}{} & Recruit diverse and creative participants. \\
    \rec{rec:diverse}{} & Recruit engaged and excited participants and facilitators. \\
    \rec{rec:vocab}{} & Evaluate domain knowledge before designing. \\
    \rec{rec:constraints}{} & Recognize workshop constraints to winnow the design space. \\
    \rec{rec:improvise}{} & Recognize tradeoffs of scripted vs improvised. \\
    \rec{rec:pilot}{} & Pilot workshops to test, evaluate, and improve methods. \\
    \hline
    \rec{rec:prepare}{} & Prepare for execution with facilitation resources. \\
    \rec{rec:materials}{} & Gather appropriate materials for workshop methods. \\
    \rec{rec:guidance}{} & Guide the workshop to foster creativity. \\
    \rec{rec:adapt}{} & Adapt facilitation to participant reactions. \\
    \rec{rec:artifacts}{} & Create artifacts --- anything not written will likely be lost. \\
    \hline
    \rec{rec:inspiring}{} & Expect rich and inspiring artifacts that warrant action. \\ 
    \rec{rec:time}{} & Allocate significant time for workshop analysis --- a day or more. \\
    \rec{rec:complement}{} & Complement workshops with traditional user-centered design methods.  \\
    \rec{rec:generative}{} & Use workshop outputs for divergent visualization design methods.  \\ 
    \rec{rec:evaluative}{} & Use workshop outputs for convergent visualization design methods.  \\
    \rec{rec:revisit}{} & Revisit workshop output and insights throughout the project. \\
    \hline
    \end{tabular}
    \caption{Summary of the workshop process recommendations.}
    \label{tab:recommendations}
\end{table}

==> tables/trash/workshops.tex <==
% \begin{table*}
%     \small
%     \centering
%     \begin{tabular}{|lllp{1cm}p{1cm}p{1cm}p{1cm}|}
%         \hline
%         \textbf{ID} & \textbf{Focus} & \textbf{Goal} & \textbf{Length (hrs)} & \textbf{Team} & \textbf{Partic. (collab)} & \textbf{Partic. (vis)} \\ \hline
%         \customlabel{\ref{pro:edina}.R}{wor:edina} & Req. & Explore possibilities for enhancing legends with visualizations & 6 & 1 & 7 & 3 \\
%         \customlabel{\ref{pro:edina}.D}{wor:edina:des} & Des. &  Candidate solutions identified and considered in light of identified requirements & 6 & 1 & --- & 3 \\   
%         \customlabel{\ref{pro:edina}.E}{wor:edina:eva} & Eval. & Presentation and evaluation of deliverables & 4 & 1 & 3? & 3  \\   
%         \hline
%         \customlabel{\ref{pro:eon}.R}{wor:eon} & Req. & Identify future opportunities for  utilising smarthome data/technologies & 6 & 3 & 5 & 0\\ 
%         \customlabel{\ref{pro:eon}.D1}{wor:eon:des1} & Des. & Develop concepts from req. workshop in an agile approach  & 4 & 2 & 0 & 6 \\
%         \customlabel{\ref{pro:eon}.D2}{wor:eon:des2} & Des. & Elicit feedback from prototypes and prioritize design improvements & 3 & 2 & 7 & 0  \\ 
%         \customlabel{\ref{pro:eon}.E}{wor:eon:eva} & Eval. & Evaluate final prototypes & 3  & 2 & 5 & 0 \\ 
%         \hline
%         \customlabel{\ref{pro:htva}.R}{wor:htva} & Req. & Identify novel visual approaches most suitable for HTA & 9 & 2 & 6 & 7 \\
%         \customlabel{\ref{pro:htva}.D}{wor:htva:des} & Des. & To further establish requirements ... to acquire feedback on initial designs  & 7 & 1 & 3 & 6 \\
%         \customlabel{\ref{pro:htva}.E}{wor:htva:eva} & Eval. & Structured evaluation against scenarios & 4 & 1 & 3 & 6 \\
%         \hline
%         \customlabel{\ref{pro:cp}.R}{wor:cp} & Req. & Identify analysis and visualization opportunities for improved profiling of cons. prog. & 2 & 7 & 10 & 0\\
%         \hline
%         \customlabel{\ref{pro:graffinity}.R}{wor:graffinity} & Req. & Explore shared user needs for visualization in retinal connectomics & 7 & 4 & 9 & 0 \\
%         \hline
%         \customlabel{\ref{pro:lineage}.R}{wor:lineage} & Req. & Understand the main tasks of psychiatric researchers & 3 & 2 & 6 & 1 \\
%         \hline
%         \customlabel{\ref{pro:updb}.R}{wor:updb} & Req. & Explore opportunities for a design study with genealogists & 3 & 1 & 7 & 3 \\
%         \hline
%         \customlabel{\ref{pro:arbor}.R}{wor:arbor} & Req. & Explore opportunities for funded collaboration between vis. and bio. & 7 x 2 & 2 & 10 & 2 \\
%         \hline
%     \end{tabular}
%     \caption{We have analyzed our 15 diverse workshops, ranging in size from 3 to 10 participants, and varying in duration from 3 hours to 2 days. This paper focuses on requirements workshops which are often used to understand domain problems and analysis needs during the formative stages of applied research collaborations.}
%     \label{tab:workshops}
% \end{table*}

\begin{table*}
    \small
    \centering
    \begin{tabular}{|ll|llll|l|lll|}
        \hline
        \textbf{ID} & \textbf{Theme} & \textbf{u} & \textbf{i} & \textbf{m} & \textbf{d} & \textbf{Focus} & \textbf{Facil.} & \textbf{Partic.} & \textbf{Hrs} \\ \hline
        \customlabel{\ref{pro:edina}.R}{wor:edina} & Explore possibilities for enhancing legends with visualizations & $\CIRCLE$ & $\Circle$ & & & Req. & 1v & 3v / 5c & 6 \\
        \customlabel{\ref{pro:edina}.D}{wor:edina:des} & Candidate solutions identified and considered in light of identified requirements & $\Circle$ & $\CIRCLE$ & $\CIRCLE$ & & Des. & 1v & 3v / 5c & 6 \\
        \customlabel{\ref{pro:edina}.E}{wor:edina:eva} & Presentation and evaluation of deliverables & $\Circle$ & $\Circle$ & $\CIRCLE$ & & Eva. & 1v & 3v / 3c & 4 \\
        \hline
         \customlabel{\ref{pro:eon}.R}{wor:eon} & Identify future opportunities for utilising smart home data/technologies & $\CIRCLE$ & $\Circle$ & & & Req. & 2v / 1p & 0v / 5c & 6 \\
        \customlabel{\ref{pro:eon}.D1}{wor:eon:des1} & Develop concepts from req. workshop in an agile approach & $\Circle$ & $\CIRCLE$ & $\Circle$ & & Des. & 2v & 6v / 0c & 4 \\
        \customlabel{\ref{pro:eon}.D2}{wor:eon:des2} & Elicit feedback from prototypes and prioritize design improvements & $\CIRCLE$ & $\Circle$ & $\CIRCLE$ &  & Des. & 2v & 0v / 7c & 3 \\
        \customlabel{\ref{pro:eon}.E}{wor:eon:eva} & Evaluate final prototypes & $\Circle$ & $\CIRCLE$ & $\CIRCLE$ & & Eva. & 2v & 0v / 5c & 3  \\
        \hline
        \customlabel{\ref{pro:htva}.R}{wor:htva} & Identify novel visual approaches most suitable for HTA & $\CIRCLE$ & $\Circle$ &  &  & Req. & 1v / 1p & 7v / 6c  & 9  \\
        \customlabel{\ref{pro:htva}.D}{wor:htva:des} & To further establish requirements ... to acquire feedback on initial designs & $\CIRCLE$  & $\Circle$ & $\CIRCLE$ &  & Des. & 1v & 6v / 3c & 7 \\
        \customlabel{\ref{pro:htva}.E}{wor:htva:eva} & Structured evaluation against scenarios & $\Circle$ & $\CIRCLE$ &  $\CIRCLE$ & & Eva. & 1v & 6v / 3c & 4  \\
        \hline
        \customlabel{\ref{pro:graffinity}.R}{wor:graffinity} & Explore shared user needs for visualization in retinal connectomics & $\CIRCLE$ & $\Circle$ & & & Req & 4v & 0v / 9c & 7 \\
        \hline
        \customlabel{\ref{pro:cp}.R}{wor:cp} & Identify analysis and visualization opportunities for improved profiling of cons. prog. & $\CIRCLE$ & $\Circle$ &  & & Req. & 2v / 1c & 0v / 10c & 7 \\
        \hline
        \customlabel{\ref{pro:lineage}.R}{wor:lineage} & Understand the main tasks of psychiatric researchers & $\CIRCLE$ & $\Circle$ &  &  & Req. & 2v & 1v / 6c & 3  \\
        \hline
        \customlabel{\ref{pro:updb}.R}{wor:updb} & Explore opportunities for a design study with genealogists & $\CIRCLE$ & $\Circle$ &  &  & Req. & 1v & 3v / 7c  & 3 \\
        \hline
        \customlabel{\ref{pro:arbor}.R}{wor:arbor} & Explore opportunities for funded collaboration between vis. and bio. & $\CIRCLE$ & $\Circle$ & & & Req & 1v / 1c & 2v / 12c & 7x2 \\
        \hline
    \end{tabular}
    \caption{Workshops that we used within each project.  We categorize workshops by how they fulfilled activities in the design activity framework~\cite{McKenna2014}: (u)nderstand user needs, (i)deate solutions, (m)ake and evaluate prototypes, as well as (d)eploy prototypes. As one workshop can influence many activities, we differentiate between explicitly focused activities ($\CIRCLE$) from more serendipitous or emergent activities ($\Circle$). This categorization reinforces the workshop focuses propesed by Goodwin et al.~\cite{Goodwin2013}: requirements (understand, ideate), design (ideate, make), and evaluation (make, ideate). We characterize workshop facilitators and participants by their affiliation as (v)isualization researchers, (c)ollaborators, or (p)rofessional facilitators.}
    \label{tab:workshops}
\end{table*}

 % & U & I & M & D & Des. & team & partic & hrs  \\
